Spin-polarized Andreev tunneling through the Rashba chain

We demonstrate that the selective equal spin Andreev reflection (SESAR) spectroscopy can be used in STM experiments to distinguish the zero-energy Majorana quasiparticles from the ordinary fermionic states of the Rashba chain. Such technique, designed for probing the p-wave superconductivity, could be applied to the intersite pairing of equal-spin electrons in the chain of magnetic Fe atoms deposited on the superconducting Pb substrate. Our calculations of the effective pairing amplitude for individual spin components imply the magnetically polarized Andreev conductance, which can be used to `filter' the Majorana quasiparticles from the ordinary in-gap states, although the pure spin current (i.e., perfect polarization) is impossible.

==> qwer <==
Modem: 517266892 (orange)

(Simon):
*) the polarization studied there concerns directions perpendicular to the direction of the applied Zeeman field. Of only Dresselhaus or Rashba SOC is present the x and y polarizations are proportional to the corresponding transverse spin polarizations. In our case polarization parallel to the field is studied, what would be easier to measure in STM experiments with the help of a ferromagnetic tip - especially the component with the same polarization as the polarizationof the STM tip. (?)

*) We agree that we propose to use the method of SESAR proposed by P. Lee to measure the spin polarization described in the paper by P. Simon to detect the Majorana states. However, here we demonstrate that the use of SESAR allows one to single out the polarization in the "z" direction of the topological states from the all the subgap states. It can be seen in Fig. 1a in paper ... that both the Majorana and ordinary states display a nonzero polarization. In contradistinction, Fig. ... of our papper shows that the transmittance for equal-spin Andreev tunneling is strongly suppressed for ordinary in-gap states and enhanced for the Majorana states (at least for one direction of the polarization).


(P. Li)
*) We demonstrate that the tunneling current is not fully spin-polarized 
*) We propose to use SESAR in STM to reveal the presence and spatial profile of the Majorana states. The aim of the paper by ... is to demonstrate that Majorana-induced SESAR can be used to create spin-polarized current. In this aspect, we demonstrate that the tunneling current is polarized, but the polarization is less than 100%.

Policzyc zmiane transmitancje calkowita i spolaryzowana w funkcji np. V_z przy przejsciu pomiedzy topo i nie-topo

Sprawdzic kierunek Rashby i ewentualnie poprawic \alpha=(0,0,alpha)


==> qwer1 <==
> Reviewer #1 (Remarks to the Author):
> 
> The manuscript claim that the selective equal-spin
> Andreev reflection spectroscopy can be used to distinguish
> the zero-energy Majorana quasiparticles from the ordinary
> fermionic states.
> However, it is hard to give this conclusion from the data
> shown in paper. The whole manuscript only gives the results
> related to Majorana quasiparticles and does not show any
> data about the ordinary state. Thus, the data is incomplete
> to support their claim. I'm also confusied by the formula of
> Eq. (6). It is very different to conventional current formula.
> The authors should show how they got the formula.
> Based on these reasons, I do not support the publication of
> this manuscript.
> 
> Reviewer #2
> 
> In this manuscript, authors study spectral functions,
> transmittances, and differential conductance of the nanoscopic
> chain of the magnetic Fe atoms deposited on the s-wave
> conventional superconductor and probed by the polarized STM
> tip. The qualitatively agreement of their theoretical results
> with the recent reported spin-polarized features in the subgap
> spectroscopy makes this study timely. Here I have the
> following comments regarding the study.
> Firstly, the present work is titled “Polarization of the
> Majorana quasiparticles in the Rashba chain”. However, this
> topic has been investigated in details in
> Ref. [PRL 108, 096802]. Furthermore, authors claim that
> “they demonstrate the selective equal-spin Andreev reflection
> (SESAR) spectroscopy can be used to distinguish the
> zero-energy Majorana quasiparticles from the ordinary
> fermionic states of the Rashba chain”. However, this point
> has been proposed in Ref. [PRL 112, 037001]. In my opinion,
> this work is a theoretical study of the STM imaging of the
> Majorana quasiparticles based on the SESAR. Authors can
> organize the results to make this point stand out.
> Secondly, in Ref. [PRL 112, 037001], where the SESAR induced
> by Majorana fermions is proposed, the 1D normal
> lead/topological superconductor junction is used to
> demonstrate the SESAR, because the Majorana fermions is
> localized in the ends of the topologicalsuperconductor.
> In Fig. 1 of the present work, however, the SESAR is
> demonstrated in the middle of the 1D topological
> superconductor probed by the STM tip, which contradicts with
> the end-localized picture of the Majorana fermions, and thus
> may causes misunderstanding. Since the two setups seem to be
> different, authors should illustrate more clearly how the
> SESAR occurs in the STM-type setup they used.
> Thirdly, in Ref. [Physica E 74, 614–624], novel signatures
> of Majorana fermions measured by means of spin-polarized STM
> has been investigated in details. Authors should cite this
> reference and explain the main similarities and differences
> between the results of the present work and those of the
> previous one, and furthermore indicate the main advances
> obtained in the present work.
> Lastly, to make the present work more self-contained and
> clearly, Some mathematical notations should be specified
> and improved. For example, the relation between the hopping
> integral t_{ij} and t should be specified; the spin index
> \alpha in caption of Fig. 5 should be replaced by \gamma,
> since \alpha has been used to denote the spin-orbital
> coupling.

